Fair $k$-Center: a Coreset Approach in Low Dimensions

Center-based clustering techniques are fundamental in some areas of machine learning such as data summarization. Generic $k$-center algorithms can produce biased cluster representatives so there has been a recent interest in fair $k$-center clustering. Our main theoretical contributions are two new $(3+\epsilon)$-approximation algorithms for solving the fair $k$-center problem in (1) the dynamic incremental, i.e., one-pass streaming, model and (2) the MapReduce model. Our dynamic incremental algorithm is the first such algorithm for this problem (previous streaming algorithms required two passes) and our MapReduce one improves upon the previous approximation factor of $(17+\epsilon).$ Both algorithms work by maintaining a small coreset to represent the full point set and their analysis requires that the underlying metric has finite-doubling dimension. We also provide related heuristics for higher dimensional data and experimental results that compare the performance of our algorithms to existing ones.

==> slindingwindow.tex <==
\section{Algorithm in the Sliding Window Setting}
    The sliding window setting introduces the additional desirable constraint that the input for the problem of interest consists of the window $W$ of the most recent data items, whereas older data are considered “stale” and disregarded by the computation.
    
    Consider a data stream $P$ of points from the metric space $(\mathcal{X},d)$. At any time $t$, let $W$ denote the set of the last $N = |W|$ points arrived, for a fixed window length $N$. In the sliding window model, for a given computational problem, we aim to develop algorithms that, at any time $t$, are able to solve the instance represented by the current window $W$, using a small working memory (possibly constant or logarithmic in $N$).
    
    Different from the streaming setting, the sliding window not only considers a new point is inserted at time $t$, but also needs to delete a point which is inserted at time $t-|W|$ from the window. Suppose that $p_t$ is the point inserted at time $t$ and the first point is $p_1$. The sliding window model aim to solve the fair $k$ center problem on the data set $W(t)=\{p_i,...,p_t\}$ where $i=\max \{1, t-|W|+1\}$. To describe this property, $\forall p\in P$ $p$ has an associated counter $TTL(p)$ which means time to live. When $p$ is inserted, let $TTL(p)=N=|W|$ and it decreases by 1 at each time step. When $TTL(p)=0$, $p$ is deleted from the sliding window. 
    
    Pellizzoni et al. \cite{pellizzoni2022k} use the coreset technique to solve the $k$ center with outliers. Some ideas in their approach can also be used to solve the fair $k$ center problem. A key point in both of Pellizzoni et al. \cite{pellizzoni2022k} and \citet{chiplunkar2020solve} is to guess the optimal value of problem on a data set. Let $d_{min}(t)$ and $d_{max}(t)$ denote the lower bound and the upper bound of the optimal value on the data set $\{p_i,...,p_t\}$ where $i=\max \{1, t-|W|+1\}$ respectively. Set a constant $\lambda\in (0,1]$, let $\delta=\frac{\epsilon}{(1+\lambda)}$. We parallelized maintain a coreset for each value $\phi$ in the following set
    $$\Gamma(t)=\{(1+\lambda)^i: \lfloor \log_{1+\lambda} d_{min}(t)/2 \rfloor \leqslant i\leqslant \lceil\log_{1+\lambda} 2d_{max}(t)/\delta\rceil\}.$$
     
    By the definition of $d_{min}(t)$ and $d_{max}(t)$, there exists a $\phi^*\in \Gamma$ satisfying $\phi^*\in [r^*_{FkC}(W(t)), (1+\lambda)r^*_{FkC}(W(t))]$. 
    
    For each value $\phi\in \Gamma$, we maintain some sets of points, called $A_\phi$, $R_\phi$ and $O_\phi$. Firstly, $A_\phi$ be the set of at most $k$ points such that $\forall x,y\in A_\phi$ $d(x,y)>2\phi$. 

    \begin{lemma}
        If $\phi\geqslant r^*_{FkC}(W(t)),$ then, $\forall x\in W(t)$ $d(x,A_\phi)\leqslant 2\phi$
    \end{lemma}
    
    
    In addition to $A_\phi$, we maintain a coreset $R_\phi\cup O_\phi$. $\forall x\in R_\phi\cup O_\phi$, it has an associated neighborhood set $N_\phi(x)$ and a $m$ dimensional vector $COLOR(x)\in \{0,1\}^m$. If  $N_\phi(x)$ contains a point from group $i$, the $i$th entry of $COLOR(x)$, $COLOR_i(x)=1$ and $Pot(x,i)$ records the newest point $\in N_\phi(x)$ from group $i$. The newest point is $p$ whose $TTL(p)$ is maximum. In our construction, each point $x\in R_\phi\cup O_\phi$ must expire before all points covered by $N_\phi(x)$ expire. When $x$ expires, we still keep the virtual point $x$ in $R_\phi\cup O_\phi$ until all points covered by $N_\phi(x)$ expire. 
    
    At time step $t$, $p_t$ arrives while $p_t'$ expires. 
    \paragraph{Handle the Insertion}
    We check whether $d(p_t,A_\phi)\leqslant 2\phi$.
    \begin{itemize}
        \item If $d(p_t,A_\phi)\leqslant 2\phi$, we select $a\in A_\phi$ such that $d(p_t,a)\leqslant 2\phi$ and $TTL(a)$ is maximum. We call $p_t$'s parent is $a$, denoted by $par(p_t)=a$. Then, we insert $p_t$ into $Y_a(\phi)$ which is an $\epsilon$ proper $(\delta\phi,1)$-net of all points whose parent is $a$. Suppose that $p_t$ is from group $i$.
        \begin{itemize}
            \item  If there exists a $x\in Y_a(\phi)$ such that $d(x,p_t)\leqslant \delta\phi$, we set $COLOR_i(x)=1$ and $Pot(x,i)=p_t$. (Note that $Pot(x,i)$ records the newest point in ball $B(x,\delta\epsilon)$ from group $i$). We call $p_t$ is attracted by $x$, denoted by $att(p_t)=x$.
            \item Otherwise, add $p_t$ into $Y_a(\phi)$. Define $COLOR_i(p_t)=1$ and $Pot(p_t,i)=p_t$.
        \end{itemize}
        \item If $d(p_t,A_\phi)> 2\phi$ and $|A_\phi|<k$, we set add $p_t$ into $A_\phi$. Set $Y_{p_t}=\{p_t\}$, $COLOR_i(p_t)=1$, and $Pot(p_t,i)=p_t$.
        \item If $d(p_t,A_\phi)> 2\phi$ and $|A_\phi|= k$, we remove $a\in A_\phi$ whose $TTL(a)$ is minimum and add $p_t$ into $A_\phi$. Then, we reset $O_\phi=O_\phi\cup Y_{a}$. In this case $\phi$ is marked as "infeasible" until the time step $t+TTL(a)$ (i.e., $\phi$ is not a feasible value before point $a$ naturally expires). All points $p$ stored whose $TTL(p)\leqslant TTL(a)$ are deleted. Finally, set $Y_{p_t}=\{p_t\}$, $COLOR_i(p_t)=1$, and $Pot(p_t,i)=p_t$.    
    \end{itemize}

    \paragraph{Handle the Deletion}
    When $p_t'$ from group $i$ expires, there are following cases ($p_t'$ may meet multiple cases):
    \begin{itemize}
        \item When $p_t'\in A_\phi$, $p_t'$ is deleted from $A_\phi$ and all points in $Y_{p_t'}(\phi)$ are moved to $O_\phi$.
        \item There exists an $a\in A_\phi$ such that $p_t'\in Y_a(\phi)$, $p_t'$ is still kept.
        \item There exists an $a\in A_\phi$ and $x\in Y_a(\phi)$ such that $p_t'=pot(x,i)$, then set $pot(x,i)=\emptyset$ and $COLOR_i(x)=0$. If $\forall i\in[1,m]$ $COLOR_i(x)=0$, $x$ is deleted from  $Y_a(\phi)$.
        \item Otherwise, $p_t'$ can be directly deleted. 
    \end{itemize}

    We now show the quality of the coreset $R_\phi\cup O_\phi$.

    \begin{lemma}
        If $\phi \geqslant r^*_{FkC}(W)$, $\phi$ is not marked as "infeasible".
    \end{lemma}
    \begin{proof}
         When $\phi$ is marked as "infeasible", by the definition of $A_\phi$. There exist at least $k+1$ points in $W$ such that the distance of any two of them is strictly greater than $2\phi$. It is impossible that using at most $k$ balls with radius $2\phi$ to cover all of these $k+1$ points. Thus $r^*_{FkC}(W)>\phi$. It is contradicted with  $\phi \geqslant r^*_{FkC}(W)$. Hence, $\phi$ is not marked as "infeasible" when $\phi \geqslant r^*_{FkC}(W)$.
    \end{proof}

    In addition, 
    \begin{lemma}\label{lem:property_of_SW}
        If $\phi \geqslant r^*_{FkC}(W)$, $\forall x\in R_\phi\cup O_\phi$, Define neighbor set $N(x,\phi)=\{p\in W: att(p)=x\}$. Then, we have the following properties: 
        \begin{enumerate}[(1)]
            \item $\forall p\in W$, there exists $x\in R_\phi\cup O_\phi$ such that $p\in N(x,\phi)$ and $d(x,p)\leqslant \delta \phi$. 
            \item If $N(x,\phi)$ contains a point from group $i$, $COLOR_i(x)=1$ and $Pot(x,i)$ records the newest point from group $i$ in $N(x,\phi)$
            \item $\bigcup_{x\in R_\phi\cup O_\phi}N(x,\phi)=W$
            \item $\forall x,y\in R_\phi\cup O_\phi$ $N(x,\phi)\cap N(y,\phi)=\emptyset$
        \end{enumerate}
    \end{lemma}
    %\begin{proof}
     %   When $\phi \geqslant r^*_{FkC}(W)$,  $\phi$ is not marked as "infeasible". Hence, there is no point $p$ expiring before $TTL(p)=0$. $\forall p\in W$
    %\end{proof}

    Thus, once $\delta\phi \leqslant \frac{\epsilon}{\alpha}r^*_{FkC}(W) $, the $R_\phi\cup O_\phi$ is an $\epsilon$-proper $(r,\alpha)-net$ of $W$. 

    To illustrate the efficiency of the update time, we now analyze the size of the coreset maintained. The important part is to analyze the number of points in $O_\phi$. Firstly, we have the following lemma:

    \begin{lemma}\label{lem:orphan}
        Recall that all parents of points in $O_\phi$ have been expired. Define $A'_\phi=\{par(x):x\in O_\phi\}$. $A'_\phi$ contains these points that were in $A'_\phi$ but have been deleted now. We have $|A'_\phi|\leqslant k$.
    \end{lemma}
    \begin{proof}
        Suppose that $A'_\phi=\{a_1,...,a_{h}\}$ and $h>k$. W.l.o.g, assume that $a_i$ is the $i$th point which expires from $W$ among  $A'_\phi$. Consider $a_1$ and $a_{k+1}$. We show that they do not co-occur in set $A_\phi$. Since each point in $\{a_1,a_2,...a_k\}$ arrives in $W$ before $a_{k+1}$, by the construction, there are two cases when $a_{k+1}$ arrives:
        \begin{itemize}
            \item $|A_{\phi}|<k $, in this case, $a_1$ have been expired and $Y_{a_1}(\phi)$ are moved to $O_\phi$. Note that by definition $\forall x\in Y_{a_1}(\phi)$, $TTL(x)<a_{k+1}$.
            \item $|A_{\phi}|=k $, in this case, $\phi$ is marked as "infeasible", $a_1$ is directly removed from $W$ and $Y_{a_1}(\phi)$ are moved to $O_\phi$. Similarly, $\forall x\in Y_{a_1}(\phi)$, $TTL(x)<a_{k+1}$.
        \end{itemize}
        Thus $a_{1}$ and $a_{k+1}$ do not co-occur in set $A_\phi$. Now consider the time that $a_{k+1}$ expires. 
        \begin{itemize}
            \item If $a_{k+1}$ expires when $TTL(a_{k+1})=0$, any point $x\in Y_{a_1}(\phi)$ has been expired because $TTL(x)<TTL(a_{k+1})$.
            \item If $a_{k+1}$ is removed from $W$ when $TTL(a_{k+1})>0$,  by the construction any point $x$ whose $TTL(x)<TTL(a_{k+1})$ is removed at the same time. Thus  all points $Y_{a_1}(\phi)$ are removed because $TTL(x)<TTL(a_{k+1})$.
        \end{itemize}
        It means that when $Y_{a_{k+1}}(\phi)$ is added into $O_{\phi}$,  $O_{\phi}$ has removed all points in  $Y_{a_{1}}(\phi)$. Hence, by definition $A'_\phi$ does not contain $a_1$, which contradicted with  $A'_\phi$ contains both $a_1$ and $a_{k+1}$. It shows that $|A'_\phi|\leqslant k$
    \end{proof}
    
    By \cref{lem:orphan}, we analyze the number of points in $R_\phi\cup O_\phi$.
    \begin{lemma}
        The window points $W$ has a finite doubling dimesion $D$. For each $\phi$, The number of points in $R_\phi\cup O_\phi$ is at most $O(k(4/\delta)^{D})$. The coreset stores $O(mk(4/\delta)^{D})$ information.
    \end{lemma}
    \begin{proof}
        $\forall a\in A_\phi$ $\forall x\in Y_a(\phi)$, we have $d(x,a)\leqslant 2\phi$, i.e., $x\in B(a,2\phi)$. Additionally, by construction $\forall x,y\in Y_a(\phi)$ $d(x,y)>\delta \phi$.
        Hence, the aspect ratio of the ball $Y_a(\phi)$ is $$\frac{\max_{x,y\in Y_a(\phi)}d(x,y)}{\min_{x,y\in Y_a(\phi)}d(x,y)}\leqslant \frac{4\phi}{\delta\phi}=\frac{4}{\delta}$$ 
        By \cref{lem:doubling}, the number of points in $Y_a(\phi)$ is at most $O((4/\delta)^{D})$. Recall that $R_\phi=\bigcup_{a\in A_\phi}Y_{a}(\phi)$ and $|A_\phi|\leqslant k$. Hence,  $|R_\phi|\leqslant O(k(4/\delta)^{D})$
        
        Similarly, we use the same way to analyze the number of points in $O_\phi$ and we know $|A'_\phi|\leqslant k$. We also have   $|O_\phi|\leqslant O(k(4/\delta)^{D})$.
        
        Finally, for each point $x$ in $O_\phi\cup R_\phi$, for each group $i$, it stores a $Pot(x,i)$. Hence, the total number of points stored is at most $O(km(4/\delta)^{D})$
    \end{proof}
    
    By construction, at each time step, when inserting a new point $p_t$ into $R_\phi\cup O_\phi$, we first check whether it is in $A_\phi$ and it takes $O(k)$ time. Then there exists $a\in A_\phi$ ($a$ could be $p_t$ itself) such that we add $p_t$ into $Y_a(\phi)$ and it takes at most $O((4/\delta)^{D})$ time. Additionally, to add $p_t$ into $A_\phi$, another $a'\in A_\phi$ could expire. We takes  $O((4/\delta)^{D})$ time to move all points in $Y_{a'}(\phi)$ from $R_\phi$ to $O_\phi$. And remove all points $x$ satisfying $TTL(x)<TTL(a')$ and it takes at most $O(km(4/\delta)^{D})$
    
    When deleting a point $p_t'$ from $R_\phi\cup O_\phi$, we first check whether it is in  $A_\phi$ and it takes $O(k)$ time. If it is in $A_\phi$, we move all points in $Y_{p_t'}(\phi)$ from $R_\phi$ to $O_\phi$. It takes at most $O((4/\delta)^{D})$ time. Additionally, when there exists $x$ such that $p_t'= Pot(x,i)$ where $p_t'$ is from group $i$, we need to delete it and check whether we need to delete $x$. The total time is at most $O(m)$.

    Overall, the total update time is at most  $O(km(4/\delta)^{D})$ for each value $\phi$. It is remaining to show the number of possible values $\phi$, i.e., the size of $\Gamma(t)$. Let $d_{max}(t)=\max_{x,y\in W}d(x,y)$ and $d_{min}(t)=\min_{x,y\in W}d(x,y)$. Obviously, $d_{min}(t)\leqslant r^*_{Fkc}(W)\leqslant d_{max}(t)$. 

    Define $\Delta(t)=\frac{d_{max}(t)}{d_{min}(t)}$. $\Delta(t)$ is called the {\em aspect ratio}. And, we have $|\Gamma(t)|=O(\log\Delta(t))$. Thus, in the sliding window model, we maintain a coreset for each value in $\Gamma(t)$. A question naturally raised: 
    
    How to maintain a coreset when $d_{max}(t)$ or $d_{min}(t)$ dynamically change?

    \subsection{Maintain $\Gamma$ under the change of $d_{max}(t)$ and $d_{min}(t)$ }
    
    Let $L=\{p_{t-k},...,p_t\}$, i.e., the last $k+1$ points in $W$. Define $LB=\min_{x,y\in L}d(x,y)/2$. Thus, $LB$ is the lower bound of $r^*_{FkC}(W)$. We also define $UB=2\max_{1<h\leqslant t}d(p_1,p_h)$ and $UB$ is the upper bound of $r^*_{FkC}(W)$.
    
    Consider 
    $$\Gamma'(t)=\{(1+\lambda)^i: \lfloor \log_{1+\lambda} LB \rfloor \leqslant i\leqslant \lceil\log_{1+\lambda} UB/\delta\rceil\}.$$
    
    When $UB$ is larger on $t+1$ time step, $\forall \phi'> \max\{\phi\in Gamma(t)\}$, we first construct a coreset for $W(t)$. Define $A_{\phi}=\{p_t\}$, $Y_{p_t}(\phi)=\{p_t\}$ and $O_\phi=\emptyset$. Additionally, find the newest point in each group $i$, let $Pot(p_t,i)=\arg \max_{x\in W(t)}TTL(x)$.  $\forall p\in W(t)$, we have $d(p,p_t)\leqslant d(p,p_1)+d(p_1,p_t)\leqslant 2d_{max}(t)<\delta \phi$. Hence, this coreset satisfies the property in \cref{lem:property_of_SW}. Currently, we have maintained a coreset for all values in $\Gamma'(t)=\{(1+\lambda)^i: \lfloor \log_{1+\lambda} LB \rfloor \leqslant i\leqslant \lceil\log_{1+\lambda} UB/\delta\rceil\}.$ We use the "handle the insertion" procedure to insert $p_{t+1}$.

    When $LB$ is smaller on $t+1$ time step, $\forall \phi'< \max\{\phi\in \Gamma(t)\}$, the distance between any two points in $\{p_{t-k},...,p_{t}\}$ is greater than $2\phi$. Thus, $\phi$ is infeasible before $p_{t-k}$ expires. We set $A_{\phi}=\{p_{t-k+1},...,p_{t}\}$, $Y_{a}(\phi)=\{a\}$ $\forall a\in A_\phi$ and $O_\phi=\emptyset$. Then, we use the "handle the insertion" procedure to insert $p_{t+1}$.

    
